Diffusion Policy Policy Optimization

We introduce Diffusion Policy Policy Optimization, DPPO, an algorithmic framework including best practices for fine-tuning diffusion-based policies (e.g. Diffusion Policy) in continuous control and robot learning tasks using the policy gradient (PG) method from reinforcement learning (RL). PG methods are ubiquitous in training RL policies with other policy parameterizations; nevertheless, they had been conjectured to be less efficient for diffusion-based policies. Surprisingly, we show that DPPO achieves the strongest overall performance and efficiency for fine-tuning in common benchmarks compared to other RL methods for diffusion-based policies and also compared to PG fine-tuning of other policy parameterizations. Through experimental investigation, we find that DPPO takes advantage of unique synergies between RL fine-tuning and the diffusion parameterization, leading to structured and on-manifold exploration, stable training, and strong policy robustness. We further demonstrate the strengths of DPPO in a range of realistic settings, including simulated robotic tasks with pixel observations, and via zero-shot deployment of simulation-trained policies on robot hardware in a long-horizon, multi-stage manipulation task. Website with code: diffusion-ppo.github.io

==> body/app_furniture_bench.tex <==
\section{Additional Details for Furniture Bench Tasks}

% \subsection{Tasks Descriptions.} 
% \begin{itemize}
%     \item  \OneLegEnv: assemble one leg of a table by placing the tabletop in the fixture corner, grasping and inserting the table leg, and screwing in the leg
%     \item \LampEnv: place the lamp base in the fixture corner, grasp, insert, and screw in the light bulb, and finally place the lamp shade
%     \item \RoundTableEnv: place a round tabletop in the fixture corner, insert and screw in the table leg, and then insert and screw in the table base.
% \end{itemize}

% \subsection{Evaluation on Furniture-Bench}

\subsection{Training details and hyperparameters for Furniture-Bench Tasks}
\label{app:furniture-hyperparameters}

With \DPPO, we pre-train a UNet-based DP with 100 DDPM denoising steps and fine-tune with 5 DDIM steps. Action chunk size $T_a=16$ is used in pre-training and then $T_a=8$ in fine-tuning. Gaussian-MLP uses $T_a=8$ in both pre-training and fine-tuning. Fine-tuning is done with 1000 parallel environments in IsaacGym~\citep{makoviychuk2021isaac}. 

% \begin{table}[H]
%     \centering
% \iftoggle{iclr}{\scriptsize}{\footnotesize}    
%     \begin{tabular}{cccc} \toprule
%     & \multicolumn{3}{c}{Task} \\
%     \cmidrule{2-4}
%     Method & One-leg & Lamp & Round-table \\
%     \hline
%     Gaussian-MLP   & 95.9  & 164.9 & 161.7  \\
%     % \hline
%     DPPO-UNet   & 193.0  & 230.2 & 250.7  \\
%     \bottomrule
%     \end{tabular}
%     \caption{Wall-clock time in seconds for a single training iteration in \textbf{FurnitureBench} tasks. Each iteration involves 1 episode (700 environment timesteps for One-leg and 1000 for Lamp and Round-table) from each of the 1000 parallelized environments running on an NVIDIA L40 GPU (700000, 1000000, 1000000 steps).}
%     \label{tab:furniture-wallclock-time}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Training details for sim-to-real transfer and hardware setup with Furniture-Bench task}
\label{app:sim2real-details}

% \textbf{Sim2Real Modifications}. To facilitate sim-to-real transfer, we add additional noise to the observations and actions in simulation training with \DPPO{}, simulating noisy real-world observations and low-level controller. Gaussian policy is trained only using observation noise; we find the action noise can break the Gaussian policy and lead to near-zero success rate in simulation. 

% \subsection{Performance in Simulation}

% \subsection{Wall-clock time}
%  Please see \cref{tab:furniture-wallclock-time} for the wall-clock time used in each of the three FurnitureBench tasks. \DPPO-UNet (five DDIM steps during sampling) takes $2.01\times$, $1.40\times$, and $1.55\times$ time compared to Gaussian-MLP, respectively.

==> body/extended_best_practices.tex <==
\section{Best Practices for \DPPO}
\label{app:implementation}

\paragraph{Fine-tune only the last few denoising steps.} Diffusion Policy often uses up to $K=100$ denoising steps with DDPM to better capture the complex data distribution of expert demonstrations. With \DPPO, we can choose to fine-tune only a subset of the denoising steps instead, e.g., the last $K'$ steps. In \cref{subsec:implementation} and \cref{sec:toy} we find this speeds up \DPPO{} training and reduces GPU memory usage without sacrificing the asymptotic performance. Instead of fine-tuning the pre-trained model weights $\theta$, we make a copy $\theta_\textsc{ft}$ --- $\theta$ is frozen and used for the early denoising steps, while $\theta_\textsc{ft}$ is used for the last $K'$ steps and updated with \DPPO.

\paragraph{Fine-tune DDIM.} Instead of fine-tuning all $K$ or the last few steps of the DDPM, one can also apply Denoising Diffusion Implicit Model (DDIM) \citep{song2020denoising} during fine-tuning, which greatly reduces the number of sampling steps $K^\textsc{DDIM} \ll K$, e.g., as few as 5 steps, and thus potentially improves \DPPO{} efficiency as fewer steps are fine-tuned. 

\begin{equation}
    x^{k-1} \sim p_\theta^\textsc{DDIM}(x^{k-1}| x^k) := \mathcal{N}( x^{k-1}; \mu^\textsc{DDIM}(x^k, \epsilon_\theta(x^k,k)), \eta \sigma_k^2\mathrm{I}), \quad k=K^\textsc{DDIM}, ..., 0. \label{eq:reverse-ddim}
\end{equation}

Although DDIM is typically used as a deterministic sampler by setting $\eta=0$ in \eqref{eq:reverse-ddim}, we can use $\eta>0$ for fine-tuning that provides exploration noise and avoids calculating Gaussian likelihood with a Dirac distribution. In practice, we set $\eta=1$ for training (equivalent to applying DDPM \cite{song2020denoising}) and then $\eta=0$ for evaluation. \emph{We reserve DDIM sampling for our pixel-based experiments and long-horizon furniture assembly tasks, where the efficiency improvements are much desired.}

% \paragraph{Denoising-dependent clipping.} Clip more for early denoising steps

\paragraph{Diffusion noise scheduling.} We use the cosine schedule for $\sigma_k$ introduced in \cite{nichol2021improved}, which was originally annealed to a small value on the order of $1E-4$ at $k=0$. In \DPPO, the value of $\sigma_k$ also translates to the exploration noise that is crucial to training efficiency. Empirically, we find that clipping $\sigma_k$ to a higher minimum value {(denoted $\sigma^\text{exp}_\text{min}$, e.g., $0.01-0.1$)} when sampling actions helps exploration (see sensitivity analysis in \cref{subsec:ablations}). Additionally we clip $\sigma_k$ to be at least $0.1$ {(denoted $\sigma^\text{prob}_\text{min}$)} when evaluating the Gaussian likelihood $\log \bar \pi_\theta(\bar a_{\bart} | \bar s_{\bart})$, which improves training stability by avoiding large magnitude.

\paragraph{Network architecture.} We study both Multi-layer Perceptron (MLP) and UNet \citep{ronneberger2015u} as the policy heads in Diffusion Policy. An MLP offers simpler setup and we find it generally fine-tunes more stably with \DPPO. Moreover, since the UNet applies convolution to the denoised action, we can pre-train and fine-tune with different action chunk size $T_a$ (the number of environment timesteps that the policy predicts future actions with), e.g., $16$ and $8$. We find that \DPPO{} benefits from pre-training with larger $T_a$ (better prediction) and fine-tuning with smaller $T_a$ (more amenable to policy gradient)\footnote{With fully-connected layers in MLP, empirically we find that using different chunk sizes for pre-training and fine-tuning with MLP leads to training instability.}.

==> body/proof.tex <==

% \subsection{Proof of \cref{prop:advantage}}
% \label{app:proof}
% \begin{proof}
% \begin{align}
%  \Exp^{(\sbar_{\bart}, \abar_{\bart}) \sim \bar\pi_{\theta_\text{old}}}\Big[
%  A^{\bar\pi_{\theta_\text{old}}}(\sbar_{\bart}, \abar_{\bart}) 
%  \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big] 
% %
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% % \underbrace{
% \big(\hat{r}(\bar s_{\bart}, \abar_{\bart}) - V^{\bar\pi_{\theta_{\text{old}}}}(\bar s_{\bart})\big)
% % }_{\hat{A}(\sbar_{\bart},\abar_{\bart})}
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big]. \\
% % &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% % \gamma^{k-1} A^{\pi_{\theta_\text{old}}}(\bar s_{\bar t(t, k=1)}, \bar a_{\bar t(t, k=1)}) 
% %  % \big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(s_t)\big)
% % \frac{
% % \bar\pi_{\theta}
% % (\abar_{\bart} \mid \sbar_{\bart})
% % }{ 
% % \bar\pi_{\theta_\text{old}}
% % (\abar_{\bart} \mid \sbar_{\bart})
% % }\Big].
% % \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% % \underbrace{
% \gammaddpm^{k} 
% \big(\hat{r}(\bar s_{\bart(t,0)}, \abar_{\bart(t,0)}) - V^{\bar\pi_{\theta_{\text{old}}}}(\bar s_{\bart(t,0)})\big)
% % }_{\hat{A}(\sbar_{\bart},\abar_{\bart})}
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} 
% \big(\hat{r}_{\bart(t, k=1)} - \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t, a_t^0]\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} 
% \big(\hat{r}_{\bart(t, k=1)} - \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t]\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k\right
% \end{align}
% \end{proof}


% % \begin{proof}
% %     $\Exp[ \Exp[f(X) | Y] g(Y)] = \Exp[ \Exp[f(X) g(Y) | Y] ]] = \Exp[f(X)g(Y)]$.
% % \end{proof}

% % \begin{theorem} Let $\bar{\gamma}(\bart) = 1$ for $\bart=\bart(t, k), k>1$, then
% % \label{theorem1}
% % \end{theorem}
% \begin{proof}

% \begin{lemma}[Tower Rule Consequence] $\Exp[ \Exp[f(X) | Y] g(Y)] = \Exp[f(X) g(Y)]$
% \end{lemma}

% % \sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t})
%  % \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k

% \begin{align}
%  % &
%  \Exp^{(\sbar_{\bart}, \abar_{\bart}) \sim \bar\pi_{\theta_\text{old}}} \Big[\big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart})\big)
%  \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big]
% &\overset{(i)}{=}\Exp\left[
% % \Exp
% \left( 
% \sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t}) 
% - \Exp \left[\sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t})\right]
% \right)
% \frac{
% \pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})}{ 
% \pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% } \right] \\
% &\overset{(i)}{=}\Exp\left[\left(
% \sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t}) 
% - \Exp \left[\sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t})\right]
% \right)\frac{
% \pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})}{ 
% \pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% } \right] \\
% % \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k\right]\\
%  &\overset{(ii)}{=}\Exp\left[
% \left( 
% \sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t}) 
% - \Exp \left[\sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t})\right]
% \right)
% \frac{
% \pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})}{ 
% \pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }
% \right] \\
% % \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k\right]\\
% &
% =\Exp\left[[A^{\pi_{\theta_\text{old}}}(\bar{o}_k, \bar{a}_k^{0}, 0) \frac{
% \pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart}
% }{ 
% \pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% } \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k\right], \\
% &=\Exp\Big[
%  \big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(s_t)\big)
% \frac{
% \pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart}
% }{ 
% \pi_{\theta_\text{old}}
% (\bar{a}_k^{t-1} \mid \bar{a}_k^t, \bar{o}_k, t)
% }\Big]
% \end{align}
% \end{proof}










% \citet{psenka2023learning} attempts to learn a value estimator that depends on both the environment state $s_t$ and the denoised action $a^k_t$ that is used in policy gradient update for the two-layer MDP, which we find leading to significant worse performance as shown in \cref{subsec:ablations}, most likely due to the difficulty of learning value based on very noisy action samples.
% Learning the \emph{state-action} value function can lead to considerably worse DDPO performance, which is also noted by \cite{psenka2023learning}, most likely due to the high stochasticity in the action

% and is justified by the following proposition demonstrating unbiasedness of our choice. \mscomment{add explanation text}
% \paragraph{Simplifying the advantage function.} Notice that the state-value function $V$ used in calculating the advantage is a function of $\sbar_{\bart(t,k)} = (s_t, a^k_t)$. However, $a^k_t$ is a noisy action sample, which can make it difficult to learn the expected future value from $\sbar_{\bart}$. Thankfully, we can use the fact that $\bar R_{\bart} = 0$ for $k > 1$ show the following:
% show that we can simply drop $a^k_t$ and use $V(s_t)$ instead of $V(\sbar_{\bart})$:
% \begin{align}
%     \bar{\gamma}\big(\bart(t,k)\big) &= \gamma^t, \gamma < 1, \\
% \text{then} \ 
%     % \bar{\gamma}(\bart(t,k))  = \begin{cases} 1 & k > 1\\
%     % \gamma^t < 1 & k = 1
%     % \end{cases}, \ \text{then} \
%     V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart}) \leftarrow \Exp\Big[\sum_{\tau(t,k) \ge \bart} \bar\gamma(\tau)\bar R(\sbar_{\tau},\abar_{\tau})\Big] 
%     % \\
%     &= \Exp\Big[\sum_{\tau(t,k) \ge \bart} \gamma^t \bar R(\sbar_{\tau},\abar_{\tau})\Big] 
%     % \quad (\text{by})
%     = \Exp\Big[\sum_{\tau(t) \ge \bart} \gamma^t  R(s_{t}, a_{t}^0)\Big] 
%     % \\
%     \rightarrow V^{\bar\pi_{\theta_{\text{old}}}}(s_t).
% \end{align}

%reward estimator $\hat{r}(\bar s_{\bart}, \abar_{\bart}) := \sum_{\tau \ge \bart} \bar \gamma$

% The proof is presented at \cref{app:poof}. Thus we can set the advantage estimator to be
% \begin{align}
%     \hat{A}(\sbar_{\bart},\abar_{\bart}) = \gammaddpm^{k}\left( \hat{r}(\bar s_{\bart}, \abar_{\bart}) - \hat{V}_{\psi}(\sbar)\right), \quad \bart = (t,k). 
% \end{align}
% We then fit a value function, $\hat{V}_{\psi}(\sbar)$, described below, and finally 

% We now apply Proximal Policy Optimization (PPO), a widely popular policy gradient method, to improve training stability and sample efficiency when optimizing \eqref{eq:dppo-objective}. It involves using the advantage function and clipping the likelihood ratio between the old and the current policy to be at most $\epsilon$ different. We can then perform multiple batch updates for each collected state-action pair.

% \begin{align}
% \nabla_\theta \cL (\pi_{\theta})= \nabla_\theta \ \mathbb{E}_{o,a \sim \pi_{\theta_\text{old}}} \ \min \left(\frac{\pi_\theta(a \mid o)}{\pi_{\theta_\text{old}}(a \mid o)} A^{\pi_{\theta_\text{old}}}(o, a), \operatorname{clip}\left(\frac{\pi_\theta(a \mid o)}{\pi_{\theta_\text{old}}(a \mid o)}, 1-\epsilon, 1+\epsilon\right) A^{\pi_{\theta_\text{old}}}(o, a)\right)
% \end{align}

% \begin{alignat}{3}
% \nabla_\theta \bar\cJ (\bar \pi_{\theta}) &= 
% \nabla_\theta \ \mathbb{E}^{(\sbar_{\bart}, \abar_{\bart}) \sim \bar\pi_{\theta_\text{old}}} \ \min \Big( &&  
% A^{\bar \pi_{\theta_\text{old}}}(\sbar_{\bart}, \abar_{\bart}) \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }, \
% % & && 
% A^{\bar \pi_{\theta_\text{old}}}(\sbar_{\bart}, \abar_{\bart})
% \operatorname{clip} \big( \frac{ 
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }, 1-\epsilon, 1+\epsilon \big) \Big),\label{allens:thing}
% \end{alignat}
% where $A^{\bar \pi_{\theta_\text{old}}}(\sbar_{\bart}, \abar_{\bart}) = \hat{r}(\sbar_{\bart}, \abar_{\bart}) - V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart})\footnote{In practice, we use Generalized Advantage Estimation [cite] that better balances variance and bias. For the ease of introducing rest of the method, we present the simpler form here.}, \ \hat{r}(\sbar_{\bart}, \abar_{\bart}) = \sum_{\tau \ge \bart} \bar\gamma(\tau)\bar R(\sbar_{\tau},\abar_{\tau})$. We also denote $\hat{r}_{\bart} = \hat{r}(\sbar_{\bart}, \abar_{\bart})$.

% = \sum_{t \ge \bart} \bar\gamma(t)\bar R(\sbar_{t},\abar_{t}) - V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart}) 

% \paragraph{Simplifying the advantage function.} Notice that the state-value function $V$ used in calculating the advantage is a function of $\sbar_{\bart(t,k)} = (s_t, a^k_t)$. However, $a^k_t$ is a noisy action sample, which can make it difficult to learn the expected future value from $\sbar_{\bart}$. Thankfully, we can use the fact that $\bar R_{\bart} = 0$ for $k > 1$ show the following:
% show that we can simply drop $a^k_t$ and use $V(s_t)$ instead of $V(\sbar_{\bart})$:
% \begin{align}
%     \bar{\gamma}\big(\bart(t,k)\big) &= \gamma^t, \gamma < 1, \\
% \text{then} \ 
%     % \bar{\gamma}(\bart(t,k))  = \begin{cases} 1 & k > 1\\
%     % \gamma^t < 1 & k = 1
%     % \end{cases}, \ \text{then} \
%     V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart}) \leftarrow \Exp\Big[\sum_{\tau(t,k) \ge \bart} \bar\gamma(\tau)\bar R(\sbar_{\tau},\abar_{\tau})\Big] 
%     % \\
%     &= \Exp\Big[\sum_{\tau(t,k) \ge \bart} \gamma^t \bar R(\sbar_{\tau},\abar_{\tau})\Big] 
%     % \quad (\text{by})
%     = \Exp\Big[\sum_{\tau(t) \ge \bart} \gamma^t  R(s_{t}, a_{t}^0)\Big] 
%     % \\
%     \rightarrow V^{\bar\pi_{\theta_{\text{old}}}}(s_t).
% \end{align}

% \begin{proposition}[Denoising-independent Advantage] Let $\bar \gamma\big(\bart(t,k)\big) = \gamma^k\bar \gamma\big(\bart(t,k=K)\big), \gamma < 1$, then 
% % Let $\bar{\gamma}(\bart) = 1$ for $\bart=\bart(t, k), k>1$, then
% \begin{align}
%  % &
%  \Exp^{(\sbar_{\bart}, \abar_{\bart}) \sim \bar\pi_{\theta_\text{old}}}\Big[
%  A^{\bar\pi_{\theta_\text{old}}}(\sbar_{\bart}, \abar_{\bart}) 
%  % \big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart})\big)
%  \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big] &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} A^{\pi_{\theta_\text{old}}}(\bar s_{\bar t(t, k=1)}, \bar a_{\bar t(t, k=1)}) 
%  % \big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(s_t)\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} 
% \big(\hat{r}_{\bart(t, k=1)} - V^{\bar\pi_{\theta_{\text{old}}}}(\bar s_{\bart(t,k=1)})\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} 
% \big(\hat{r}_{\bart(t, k=1)} - \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t, a_t^0]\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% % \\
% % &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% % \gamma^{k-1} 
% % \big(\hat{r}_{\bart(t, k=1)} - \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t]\big)
% % \frac{
% % \bar\pi_{\theta}
% % (\abar_{\bart} \mid \sbar_{\bart})
% % }{ 
% % \bar\pi_{\theta_\text{old}}
% % (\abar_{\bart} \mid \sbar_{\bart})
% % }\Big].
% % \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k\right
% \end{align}
% \label{prop:advantage}
% \end{proposition}
% But we are learning $V(s_t) \leftarrow \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t, a_t^0]$ instead of $V(s_t, a_t^0)$

% The proof is presented at \cref{app:proof}. 
% This means we can simply use the advantage at $k=1$ for all $t$, and since the state at $k=1$, $\bar s_{\bar t(t, k=1)} = (s_t, $

% Now $V^{\bar\pi_{\theta_{\text{old}}}}$ does not depend on $a_t^k$, or $k$, and we can use it for all $K$ steps at some $t$.
% Effectively we do not apply additional discount  
% % $\bar{\gamma}(\bart) = 1$ 
% for steps $k > 1$, which should not hinder convergence since we do not need to fine-tune very long denoising process (as explained in \cref{subsec:implementation}) and we are still applying $\gamma < 1$ for $k=1$ at all $t$.



% This also leads this following simplified form of advantage estimator:
% First, using the fact that $\bar R(\bart)=0$ at $k > 0$, 
% \mscomment{explain that this b/c rewards are zero except for those times}
% Now, we observe
% \begin{proposition}[Denoising-independent Advantage] 
% Let $\gammaddpm \in (0,1)$ be the diffusion discount, then 
% Let $\bar \gamma\big(\bart(t,k)\big) = \gamma^k\bar \gamma\big(\bart(t,k=K)\big), \gamma < 1$, then 
% Let $\bar{\gamma}(\bart) = 1$ for $\bart=\bart(t, k), k>1$, then
% \begin{align}
 % &
 % \Exp^{(\sbar_{\bart}, \abar_{\bart}) \sim \bar\pi_{\theta_\text{old}}}\Big[
 % A^{\bar\pi_{\theta_\text{old}}}(\sbar_{\bart}, \abar_{\bart}) 
 % \big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(\sbar_{\bart})\big)
%  \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big] 
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} A^{\pi_{\theta_\text{old}}}(\bar s_{\bar t(t, k=1)}, \bar a_{\bar t(t, k=1)}) 
%  % \big(\hat{r}(\sbar_t, \abar_t) - V^{\bar\pi_{\theta_{\text{old}}}}(s_t)\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% \sbar_{\bart}, \abar_{\bart(t,k)}
% =\Exp^{(\cdot) \sim \bar\pi_{\theta_\text{old}}}\Big[
% % \underbrace{
% \big(\hat{r}(\bar s_{\bart}, \abar_{\bart}) - \gammaddpm^{k} V^{\bar\pi_{\theta_{\text{old}}}}(\bar s_{\bart(t,0)})\big)
% % }_{\hat{A}(\sbar_{\bart},\abar_{\bart})}
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} 
% \big(\hat{r}_{\bart(t, k=1)} - \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t, a_t^0]\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \\
% &=\Exp^{(\sbar_{\bart}, \abar_{\bart(t,k)}) \sim \bar\pi_{\theta_\text{old}}}\Big[
% \gamma^{k-1} 
% \big(\hat{r}_{\bart(t, k=1)} - \Exp^{\bar \pi}[\hat{r}_{\bart(t,k=1)} | s_t]\big)
% \frac{
% \bar\pi_{\theta}
% (\abar_{\bart} \mid \sbar_{\bart})
% }{ 
% \bar\pi_{\theta_\text{old}}
% (\abar_{\bart} \mid \sbar_{\bart})
% }\Big].
% \big{|} \bar{a}_k^{t-1},\bar{a}_k^{t},\bar o_k\right
% \end{align}
% \label{prop:advantage}
% \end{proposition}
% \vspace{-10pt}
% The proof is shown at \cref{app:proof}. 
